Unveiling Cognitive Constraints in Language Production: Extracting and Validating the Active Ego Network of Words

The "ego network of words" model captures structural properties in language production associated with cognitive constraints. While previous research focused on the layer-based structure and its semantic properties, this paper argues that an essential element, the concept of an active network, is missing. The active part of the ego network of words only includes words that are regularly used by individuals, akin to the ego networks in the social domain, where the active part includes relationships regularly nurtured by individuals and hence demanding cognitive effort. In this work, we define a methodology for extracting the active part of the ego network of words and validate it using interview transcripts and tweets. The robustness of our method to varying input data sizes and temporal stability is demonstrated. We also demonstrate that without the active network concept (and a tool for properly extracting the active network from data), the "ego network of words" model is not able to properly estimate the cognitive effort involved and it becomes vulnerable to the amount of data considered (leading to the disappearance of the layered structure in large datasets). Our results are well-aligned with prior analyses of the ego network of words, where the limitation of the data collected led automatically (and implicitly) to approximately consider the active part of the network only. Moreover, the validation on the transcripts dataset (MediaSum) highlights the generalizability of the model across diverse domains and the ingrained cognitive constraints in language usage.

==> acks.tex <==
% !TEX root = manuscript.tex

This work was partially supported by SoBigData.it. SoBigData.it receives funding from European Union – NextGenerationEU – National Recovery and Resilience Plan (Piano Nazionale di Ripresa e Resilienza, PNRR) – Project: “SoBigData.it – Strengthening the Italian RI for Social Mining and Big Data Analytics” – Prot. IR0000013 – Avviso n. 3264 del 28/12/2021. 
%
C. Boldrini was also supported by PNRR - M4C2 - Investimento 1.4, Centro Nazionale CN00000013 - "ICSC -National Centre for HPC, Big Data and Quantum Computing" - Spoke 6, funded by the European Commission under the NextGeneration EU programme.


==> part1_v0.tex <==
% !TEX root = manuscript.tex
%\vspace{-5pt}

\subsection{Preliminaries}
\label{sec:preliminaries}

Before describing our method for building the ego network of words, we introduce here the notation used in the section. 
%
We denote an ego with the letter $e$, where the ego is the speaker (MediaSum) or user (Twitter) in our datasets for whom we want to extract the ego network of words. After the cleaning process discussed in Section~\ref{sec:dataset}, for each ego $e$ we end up with a tuple (i.e., an ordered sequence) of tokens, which we denote with $\mathcal{T}_e$. Note that the tokens in $\mathcal{T}_e$ are generally not unique. In computational linguistics, the term \emph{type} denotes the class of all tokens term containing the same character sequence. In other words, the set of types corresponds to the set of distinct tokens or, slightly simplifying, a type is a word and its occurrences are tokens. For example, in the sentence \emph{a rose is a rose is a rose}, there are eight tokens but only three types. In this paper, for the sake of simplicity, we use the terms \emph{type} and \emph{word} interchangeably. Similarly, tokens may be also called \emph{occurrences}. In the following, we denote the set of unique words as $\mathcal{W}_e$. In the rest of the section, when there is no risk of ambiguity, we will drop the subscript $e$ from our notation: in that case, all the variables discussed will be referred to the same tagged ego $e$.

\subsection{Method for building an ego network of words}

We call $\mathcal{W}(e)$ the multiset containing the sequence of words of a given ego $e$ obtained in the previous section. $\mathcal{W}_u(e)$  is the set containing the unique words of the same ego. Ego networks of words are used to hierarchise the words used by a given person based on their frequency. Hence, each word from $\mathcal{W}_u(e)$ is assigned to one of the $\tau^{(e)}$ rings $r_1$, $r_2$, $\ldots$ , $r_{\tau^{(e)}}$, knowing that $r_1$ (the innermost ring) contains the most frequent words  and that $r_{\tau^{(e)}}$  (the outermost ring) contains the least used words. The set of words assigned to the ring $r_i$ is called $\mathcal{W}_u(e,r_i)$ such that :


\begin{equation}
    \begin{cases}
        %\mathcal{W}_u(e,r_i) \bigcap \mathcal{W}_u(e,r_j) = \emptyset, \forall i,j \in [1,\tau^{(e)}], i \neq j \\
        
        \mathcal{W}_u(e) = \bigcup_{i=1}^{\tau^{(e)}} \mathcal{W}_u(e,r_i)\\
        |\,\mathcal{W}_u(e)\,| = \Sigma_{i=1}^{\tau^{(e)}} |\,\mathcal{W}_u(e,r_i)\,|
    \end{cases}
    \label{eq:stability-eq1}
\end{equation}

The ego network can also be studied from a cumulative perspective with  concentric layers $l_1$, $l_2$, $\ldots$ , $l_{\tau^{(e)}}$, the layer $l_i$ containing all the ring $r_j$ where $j \leq i$.  The set of words assigned to the layer $l_i$ is called $\mathcal{W}_u(e,l_i)$ such that: 
\begin{equation}
    \mathcal{W}_u(e,l_i) = \bigcup_{j=1}^{i} \mathcal{W}_u(e,r_j)
\end{equation}. 

It implies that the innermost layer $l_1$ is equivalent to $r_1$ and the outermost layer $l_{\tau^{(e)}}$ contains all the words of the ego network:
\begin{equation}
    \mathcal{W}_u(e,l_1)=\mathcal{W}_u(e,r_1)
\end{equation}
\begin{equation}
    \mathcal{W}_u(e,l_{\tau^{(e)}})=\mathcal{W}_u(e)
\end{equation}

%In the following parts of the paper, we will refer to the circles (or layers) as $\mathcal{L}_i^{(e)}$ where $e$ is the corresponding ego network of word and $i$ the rank of the circle (from 1, the innermost circle to $\tau^{(e)}$ the outermost one). Since we will not use the time component in this study the frequency simply corresponds to the number of word occurrences. 
To find the best natural grouping of words we use the Mean Shift~\cite{fukunaga1975estimation} algorithm, which is able, in contrast to Jenks~\cite{jenks1977optimal} or K-Means~\cite{macqueen1967some}, to automatically select $\tau^{(e)}$ the optimal number of groups to be found. Clustering on a unidimensional variable is equivalent to dividing the occurrences into mutually exclusive intervals.
The Mean Shift algorithm detects clusters that correspond to local maxima of an estimated density function of word frequencies. This function is obtained with the kernel density estimation for which the sensibility is set with a fixed parameter called the bandwidth. We apply a preliminary log-transformation to frequencies in order to compress high values and ensure that the same bandwidth setting allows peak detection for both the high and low frequency parts of the distribution
\footnote{Applying a log-transformation to word frequencies is a common thing in psychological research when studying the associated cognitive processes~\cite{brysbaert2018word}.}.
The obtained clusters of words correspond to the $\tau^{(e)}$ rings of the newly built ego network of words $e$, $r_1$ being the cluster containing the most frequent words and $r_{\tau^{(e)}}$ the one containing the least frequent words.

\subsection{Full vs active ego networks}

The distribution of the number of circles obtained our datasets is shown in Figure~\ref{fig:nb-circles-full}. We can observe that the obtained ego networks of words have a very low number of circles (the most frequent case is two) compared with the ego networks of words in previous work (usually between five and seven circles~\cite{ollivier2020,ollivier2022}). Note that the Twitter datasets used here are \emph{the same} as those in ~\cite{ollivier2020,ollivier2022} except for the timeline length considered (much larger, in this work). As we can observe in Figure~\ref{fig:occ-vs-layers} ego networks with  one or two circles are also the biggest ego network (\textit{i.e.} with the largest number of unique words $|\,\mathcal{W}_u(e)\,|$). This seems to suggest that, when considering larger textual inputs, the ego network model loses its finer discriminative power. Indeed, a two-circle ego network simply separates the most used words from the least used words. 

However, this finding is not unexpected: in the social ego network case, the theory distinguishes between the \emph{full} and \emph{active} ego network, stating that only the relationships in the active part are actually consuming cognitive resources. The conventional cut-off point, as stated in \cite{dunbar1998social}, is for the social relationship to involve interactions at least once a year, which, in Western societies corresponds to at least exchanging Christmas/birthday wishes. While this cut-off point could be obtained with anthropological common sense for social ego networks, it is difficult to come up with a similar rule of thumb for the ego networks of words, which are less rooted in everyday experiences. Hence, in this work, we set out to design a methodology to automatically extract the cut-off point in the ego networks of words.



\begin{figure}[h]
\centering
\begin{minipage}{.48\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/nb-circles-full.pdf}\vspace{-8pt}
  \captionof{figure}{Distribution of $\tau^{(e)}$}
  \label{fig:nb-circles-full}
\end{minipage} %
\hspace{5pt}
%
\begin{minipage}{.48\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/occ-vs-layers.pdf}\vspace{-8pt} % update figure 
  \captionof{figure}{$\tau^{(e)}$ vs $|\,\mathcal{W}_u(e)\,|$ (MediaSum)}
  \label{fig:occ-vs-layers}
\end{minipage}\vspace{-10pt}
\end{figure}

\subsection{Extracting the active ego network \label{sec:active-egonet}}

The idea behind an ego network is that all the words it contains should be actively used, even those in the outermost circle. If we let a person speak, we notice that from a certain point on the frequency of appearance of a new word decreases rapidly: a specific number of words is sufficient for this person to express himself. This quantity is the maximum number of actively used words. We can observe this phenomenon in Figure~\ref{fig:saturation-curve1}, where the number of words (y-axis) required to obtain a given number of unique words (x-axis) is plotted for a single speaker in the Mediasum dataset. We can observe two regimes. In a first phase, the number of additional word occurrences needed to discover a new word is stable (in other words, the slope of the line is constant). After the cut-off point, the slope changes.
%then it grows rapidly past a inflection point.
We will call this curve the \emph{saturation curve}. We argue that the active part of the ego network ends at the inflection point of the saturation curve. We call $W_u^{active}$ the number of unique words at that point of the curve, and $W_u^{full}$ the number of unique words at the rightmost part of the curve. If our intuition is confirmed, the well-known layered ego network structure would emerge by considering only words in the first regime of the saturation curve when computing the ego network. Indeed, this is confirmed in Section~\ref{sec:cutoff-results}.

Note that sometimes the textual data for one ego is not large enough for the ego network to reach any cut-off point (Figure~\ref{fig:saturation-curve2}). In this case, there is no need to reduce the size of the ego network.

%If we reach it, then we can just keep the corpus part needed to obtain that maximum number of active words. That is the rationale of the method explained in the next section.

\begin{figure}[h]
\centering
\begin{minipage}{.48\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/saturation-curve1.pdf}\vspace{-8pt}
  \captionof{figure}{Non-linear saturation curve.}
  \label{fig:saturation-curve1}
\end{minipage} %
\hspace{5pt}
%
\begin{minipage}{.48\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/saturation-curve2.pdf}\vspace{-8pt}
  \captionof{figure}{Linear saturation curve.}
  \label{fig:saturation-curve2}
\end{minipage}\vspace{-10pt}
\end{figure}

%First, the size of the ego network grows linearly, then after a bending point,  then the ego networks needs more and more word occurrences in the corpus to grow by one word.\\

\subsubsection{Methodology \label{sec:methodology}}

The methodology to obtain the cut-off point $W_u^{active}$ is illustrated in Figure~\ref{fig:methodology-recurs} and detailed in Algorithm~\ref{alg:cut-off}. 
To clarify the formulas in the following sections, we simplify the notation of the number of unique words in an ego network: $w_u = |\mathcal{W}_u(e)|$ at any point of the curve. For the ego network $e$, the two dimensional coordinates of the curve on the interval $[0,w_u]$ are symbolized by $x_{[0,w_u]}$ and $y_{[0,w_u]}$.
%In Algorithm~\ref{alg:cut-off} the main function \textsc{FindCutOff} is recursive: if the saturation curve is linear 
Algorithm~\ref{alg:cut-off} describes how the cut-off point is found recursively:
\begin{enumerate}
  \item If the saturation curve is linear
  \footnote{
  We use Lasso\cite{tibshirani1996regression} to determine if the curve described by $x_{[0,w_u]}$ and $y_{[0,w_u]}$ is linear. We define four polynoms features $<x_1,x_2,x_3,x_4>$ (degree one to degree four), reduced and centered, based on $x_{[0,w_u]}$. Additionally to the sum of square errors, Lasso adds a penalty $\lambda \Sigma_{i=1}^4 |\sigma_i|$ where $\lambda$ controls the impact of the penalty and $\sigma_i$ is the linear coefficient associated to $x_i$. Lasso has the particularity to reduce to 0 an increasing number of feature coefficients when $\lambda$ grows. It allows indirectly to select the best feature. If $\sigma_1$ is the last non-zero coefficient when $\lambda$ grows, it means that $x_1$ is the most suitable feature and thus the curve is linear.}
  %The objective function is $\min\limits_{\sigma} = \frac{1}{2 \times w_u} \Sigma_{i=1}^{4} || \sigma x - x_e[0,w_u] ||^2_2 - \lambda |\sigma|_1 $ where 
  on $[0,w_u^{full}]$ then the algorithm stops, the maximum number of active words is not reached ($w_u^{out} \gets W_u^{full}$). If not, the curve exhibits an inflexion point that should be found.
  \item We select $w_u^{new}$ such that the sum of square of two linear models fitted on intervals $[0,w_u^{new}]$ and $[w_u^{new},W_u^{full}]$ is the lowest.
  \item If the saturation curve is linear enough on $[0,w_u^{new}]$, then $w_u^{out} \gets w_u^{new}$. If not we repeat step 2 on interval $[0,w_u^{new}]$ to update $w_u^{new}$ with a lower value until $[0,w_u^{new}]$ is considered as linear.
  
\end{enumerate}




%on interval $[0,\mathcal{W}_u^{full}]$, then the algorithm stops and the maximum number of active words is not reached ($w_u^{out} = W_u^{full} \leq W_u^{active}$). If not, we fit a two segments polyline (Algorithm~\ref{alg:break-point}) to detect two phases of the saturation curve and call \textsc{FindCutOff} again on the interval of first phase we just found. When that first phase is linear enough, we stop and consider that the saturation point is reached ($w_u^{out} = W_u^{active} < W_u^{full}$). 
%\footnote{In Algorithms \ref{alg:linear} and \ref{alg:break-point} we implicitly consider that the fitting are made on the saturation curve (\textit{i.e.} the x-axis being $w_u$ and the y-axis being $|\mathcal{W}(e)|$).} 
%We call $w_u^{sat}$ the number of unique words at the saturation point, and $w_u^{full}$ the number of unique words in the full ego network.

%\begin{enumerate}
%  \item Verify if the saturation curve is linear. If so, then the algorithm stops and the maximum number of active words is not reached ($w_u^{full} \leq w_u^{sat}$), jump to point four. If not, there is a saturation point to find ($w_u^{full} > w_u^{sat}$), we can jump to point two.
%  \item We divide the curve in two at point $w$ (a given number of unique words). We fit two linear models on both intervals $[0,w]$ and $[w,w_u^{sat}]$. We select $w$ such that the sum of squared errors of the composed model is the lowest.
%  \item We keep the first interval $[0,w]$ of the saturation curve and test if this part is linear enough (repeat step 1 with $w_u^{full} \gets w$).
%  \item We build the ego network whose size is $w_u^{out} \gets w_u^{full}$.
%\end{enumerate}

%\greybox{\textbf{Verifying if the saturation curve is linear}
%\begin{enumerate}
%    \item $w_u$: number of unique word, $|\,\mathcal{W}(e)\,|$: number of word occurrences
%    \item $<w_u^1, w_u^2, w_u^3, w_u^4>$ are the polynomial features, center and reduced.
%    \item Train a Lasso model, with a L1 penalty coefficient $\lambda$ as input, and four feature coefficients $\alpha_1$, $\alpha_2$, $\alpha_3$, $\alpha_4$ as output.
%    \item Select the feature $w_u^i$ with the last non-zero coefficient $\alpha_i$ when $\lambda$ grows.
%    \item If the feature is $w_u^1$, then we consider the saturation curve as linear.
%\end{enumerate}
%}

%We fit the curve with a linear combination of polynoms of degree 1, 2, 3 and 4.\\
%Use lasso to select the polynom degree that fits the best to the curve.\\
%If the 1 degree is the best fit, then we consider that it is linear \\
%If the curve is not linear, then we try to find the linear first phase

\begin{algorithm}
\caption{Finds the cut-off point of a saturation curve}\label{alg:cut-off}

 \hspace*{\algorithmicindent} \textbf{Input: } $x_{[0,w_u^{full}]}$ and $y_{[0,w_u^{full}]}$ the coordinates of the saturation curve of ego network $e$ on the interval $[0,w_u^{full}]$.\\
  \hspace*{\algorithmicindent} \textbf{Output: } $w_u^{out}$ the cut-off point.\\
 %\hspace*{\algorithmicindent} \textbf{Output: } $w_u^{out}$ the cut-off point that delimits the active part of the saturation curve $[0,w_u^{out}]$\\

\begin{algorithmic}
\State $w_u^{out} \gets \Call{RecursiveCutOff}{w_u^{full}}$
\State
\Function{RecursiveCutOff}{$w_u^{in}$}
\If{\Call{IsLinear}{$w_u^{in}$}}
    \State \Return $w_u^{in}$
\Else
    \State $w_u^{new} \gets $ \Call{FindPolylineBreak}{$w_u^{in}$}
    \State \Return \Call{RecursiveCutOff}{$w_u^{new}$}
 \EndIf
\EndFunction
\State
%\caption{to check if the saturation is linear on interval $[0,w_u]$}\label{alg:linear}
\Function{IsLinear}{$w_u^{in}$}
    \State $\lambda \gets 0$ \Comment{Penalty coefficient of lasso regression}
    \State $<x_1,x_2,x_3, x_4>$ \Comment{Polynom. feat. based on $x_{[0,w_u^{new}]}$, center and reduced}
    \State $<\sigma_1, \sigma_2, \sigma_3, \sigma_4>$ \Comment{Lasso coefficient associated to the features}
    \State
    \While{\Call{CountNonZero}{$<\sigma_1, \sigma_2, \sigma_3, \sigma_4>$} $>1$}
        \State $\lambda \gets \lambda + \delta$
        \State $<\sigma_1, \sigma_2, \sigma_3, \sigma_4> \gets$ \Call{Lasso}{$x_{[0,w_u^{in}]}$,$y_{[0,w_u^{in}]}$,$<x_1,x_2,x_3,x_4>$,$\lambda$}
    \EndWhile
    \If{$\sigma_1 \neq 0$}
    \State \Return True
    \Else
    \State \Return False
    \EndIf
\EndFunction
\State
%\caption{to find the best break point of a 2-segments polyline fit}\label{alg:break-point}
\Function{FindPolylineBreak}{$w_u^{in}$}
    \State \Var{best_$w_u^{new}$} $\gets 1$
    \State \Var{lowest_ss} $\gets +\infty$
    \For{$w_u^{new} \in \llbracket 1,w_u^{in}-1 \rrbracket$}
        \State \Var{ss$_1$} $\gets$ \Call{LinearFit}{$x_{[0,w_u^{new}]}$,$y_{[0,w_u^{new}]}$}
        \State \Var{ss$_2$} $\gets$ \Call{LinearFit}{$x_{[w_u^{new},w_u^{in}]}$,$y_{[w_u^{new},w_u^{in}]}$}
        \If{\Var{ss$_1$}+\Var{ss$_2$}$<$\Var{lowest_ss}}
            \State \Var{lowest_ss} $\gets$ \Var{ss$_1$}+\Var{ss$_2$}
            \State \Var{best_$w_u^{new}$} $\gets$ $w_u^{new}$
        \EndIf
    \EndFor
    \State \Return \Var{best_$w_u^{new}$}
\EndFunction
 \State
\end{algorithmic}
\end{algorithm}

\begin{figure}[h]
    \begin{center}
        \includegraphics[scale=.4]{figures/methodology-recurs.pdf}%\vspace{-5pt}
        \caption{Algorithm for detecting the saturation point.}
        \label{fig:methodology-recurs}\vspace{-30pt}
    \end{center}
\end{figure} 

\subsection{Stability}

The approximation of the size of the active ego network $W_u^{active}$ should be stable over time and specific to each person. 
%It means that on a theoretical infinite saturation curve, \textsc{FindCutOff}($[0,w_u^{in}]$) should return $w_u^{out}=w_u^{in}$ when $w_u^{in} \in [0,W_u^{active}]$ and $w_u^{out}=W_u^{active}$ when $w_u^{in} \in [W_u^{active},+\infty]$.
It means that on a theoretical infinite saturation curve, \textsc{RecursiveCutOff}($w_u^{in}$) should return $w_u^{out}=W_u^{active}$ when $w_u^{in} \geq W_u^{active}$. In this case, we can approximate $W_u^{active}$ with $w_u^{out}$. When $w_u^{in} < W_u^{active}$ (which is the case where the saturation curve has no inflexion point), the algorithm shall simply return $w_u^{out} = w_u^{in}$. 

%if we had calculated the saturation curve with more words (\textit{i.e.} a bigger $|\,w_u^{full}\,|$), the bending point should remain the same. We want to verify if our algorithm verifies that stability constraint. 
To prove that our algorithm respects that ideal behaviour, we first calculate $W_u^{out}$ the output of the algorithm calculated with the full curve of a given user:
\begin{equation}
    W_u^{out} \gets \CUTOFF(W_u^{full})
\end{equation}
If the curve contains a saturation point, then $W_u^{out} = W_u^{active}$, if not then $W_u^{out} < W_u^{active}$.
%, and $y_{sat}$ and the size of the corpus (number of word occurrences) needed obtain $x_{sat}$ unique words. 
%We select a subpart of the curve in the interval $[0,x_{in}]$ as input to our algorithm, and we obtain an estimation of saturation point at $x_{out}$. In the ideal case, $x_{out}$ should follow the behaviour:
%\begin{equation}
%    \begin{cases}
%        w_u^{out}=w_u^{in} \;\;\;\text{for}\;\;\;  \in [0,w_u^{sat}] \\
%        w_u^{out}=w_u^{sat} \;\;\;\text{for}\;\;\; x \in [x_{sat},+\infty]
%    \end{cases}
%    \label{eq:stability-eq1}
%\end{equation}
In order to compare the results obtained with various scales, we use the ratio $\frac{w_u^{out}}{W_u^{out}}$. As stated above $w_u^{out}$ should verify the following conditions:

\begin{equation}
    \begin{cases}
        \cfrac{w_u^{out}}{W_u^{out}}=\cfrac{w_u^{in}}{W_u^{out}} \;\;\;\text{when}\;\;\; \cfrac{w_u^{in}}{W_u^{out}} \in [0,1]\\
        \cfrac{w_u^{out}}{W_u^{out}}=1 \;\;\;\text{when}\;\;\; \cfrac{w_u^{in}}{W_u^{out}} \in [1,+\infty]
    \end{cases}
    \label{eq:stability-eq2}
\end{equation}

We confirm with the empirical results in Fig~\ref{fig:stability} that the behavior of the algorithm is close to the ideal case in every dataset despite some noise due to a lower number of ego networks in the NYT journalists and science writers dataset.
%We can observe a little bump when $\cfrac{x_{out}}{x_{sat}}$ is slightly superior to $1$. We can explain this phenomenon because because we feed the algorithm with the saturation curve at between the interval $[0,x_{sat}+\epsilon]$. On this interval, the saturation curve only starts its inflexion, which is not yet detected. Once $\epsilon$ and the second phase is large enough to be detected, the algorithm gets very close to the ideal case.

\begin{figure}[h]
    \begin{center}
        \includegraphics[scale=.4]{figures/stability}%\vspace{-5pt}
        \caption{The stability of the algorithm is close from the ideal case.}
        \label{fig:stability}
    \end{center}
\end{figure} 

\subsection{Temporal stability of the active network size}

The temporal evolution of the size of the active network is important because it allows us to measure if the cognitive ability to add words to one's active vocabulary evolves over time. To evaluate the temporal evolution of this value, we change the index of the sequence of words $w_0,w_1,\cdots,w_n$ from which we start build the saturation curve. This shift $\delta$ in the considered word sequence is not measured properly with any time unit but simply as the number of words skipped, such that the new word sequence is $w_\delta,w_{\delta+1},\cdots,w_n$. Based on this updated sequence of word, we build a new saturation curve, from which we extract an active network size $W_u^{active}(\delta)$ (Figure~\ref{fig:temp-shift-stability-method}). In order to evaluate the variation of this value, we consider the ratio $\frac{W_u^{active}(\delta)}{W_u^{active}(0)}$. We see in Figure~\ref{fig:temp-shift-stability-res} that this ratio is stable when $\delta$ grows independantly of the dataset. It means that the active network size of an individual ego network is also stable. This legitimizes our hypothesis that the size and internal structure of the ego network are bound by cognitive constraints that are applied at different intensities depending on the individual, but which are themselves stable over time. 

\begin{figure}[h]
    \begin{center}
        \includegraphics[scale=.4]{figures/temp-shift-stability-method.pdf}%\vspace{-5pt}
        \caption{}
        \label{fig:temp-shift-stability-method}
    \end{center}
\end{figure} 

\begin{figure}[h]
    \begin{center}
        \includegraphics[scale=.6]{figures/temp-shift-stability-res.pdf}%\vspace{-5pt}
        \caption{}
        \label{fig:temp-shift-stability-res}
    \end{center}
    \caption{Stability }
\end{figure} 

\subsection{Results \label{sec:cutoff-results}}

The distribution of circles of the newly built ego networks of words can be seen in Fig~\ref{fig:nb-circles-active}. Limiting the size of the ego network to the maximum number of actively used words shifts the mode from two circles to four and five circles, for all datasets. These results validate our methodology. In the next section, we will study the structural properties of these ego networks of words.

\begin{figure}[h]
    \begin{center}
        \includegraphics[scale=.5]{figures/nb-circles-active.pdf}%\vspace{-5pt}
        \caption{Effects of the recursive cut on the distribution of the number of circles.}
        \label{fig:nb-circles-active}
    \end{center}
\end{figure} 

==> part1_v1.tex <==
% !TEX root = manuscript.tex
%\vspace{-5pt}

\subsection{Preliminaries}
\label{sec:preliminaries}

Before describing our method for building the ego network of words and extracting its active part, we introduce here the notation used in the section (also summarised in Table~\ref{tab:notation}). 
%
We denote an ego with the letter $e$, where the ego is the speaker (MediaSum) or user (Twitter) in our datasets for whom we want to extract the ego network of words. After the cleaning process discussed in Section~\ref{sec:dataset}, for each ego $e$ we end up with a tuple (i.e., an ordered sequence) of tokens~\cite{mogotsi2010christopher}, which we denote with $\mathcal{T}_e$. Note that the tokens in $\mathcal{T}_e$ are generally not unique. In computational linguistics, the term \emph{type} denotes the class of all tokens containing the same character sequence~\cite{mogotsi2010christopher}. In other words, the set of types corresponds to the set of distinct tokens or, slightly simplifying, a type is a word and its occurrences are tokens. For example, in the sentence \emph{a rose is a rose is a rose}, there are eight tokens but only three types. In this paper, for the sake of simplicity, we use the terms \emph{type} and \emph{word} interchangeably. Similarly, tokens may be also called \emph{occurrences}. In the following, we denote the tuple of unique words in an ego network as $\mathcal{W}_e$. Please note that both $\mathcal{T}_e$ and $\mathcal{W}_e$ are ordered sequences, where the order is defined by the appearance in the ego's timeline in chronological order. The relationship between tokens and words is illustrated below: FIG TO BE ADDED
So, if we observe the first $n$ tokens in the ego's timeline, we will get exactly $n$ token but at most $n$ unique words. We denote with $\mathcal{T}_e^n$ and $\mathcal{W}_e^n$ the tuples of tokens and unique words, respectively, observed up to $n$. 

In the rest of the section, when there is no risk of ambiguity, we will drop the subscript $e$ from our notation: in that case, all the variables discussed will be referring to the same tagged ego $e$.

% \usepackage{booktabs}
\begin{table}[]
\centering
\begin{tabular}{@{}ll@{}}
\toprule
\textbf{Symbol}     & \textbf{Description}         \\ \midrule
$\mathcal{T}_e$     & tuple of tokens, i.e., sequence of words ego $e$ has used  \\
$\mathcal{W}_e$     & tuple of unique words used by ego $e$        \\
$\mathcal{T}_e^n$   & $\mathcal{T}_e$ cut at the $n$-th token   \\
$\mathcal{W}_e^n$   & unique words in $\mathcal{T}_e^n$\\
$\tau_e$            & optimal number of circles           \\
$r_i$                & $i$-th ring of the ego network        \\
$l_i$                & $i$-th layer of the ego network       \\
$\mathcal{W}_{e,r_i}$ & unique words assigned to ring $r_i$ \\
                    % &                                     \\
                    % &                                     \\
                    % &                                     \\
                    % &                                     \\
                    % &                                     \\ 
\bottomrule
\end{tabular}
\caption{Summary of notation used in the paper.}
\label{tab:notation}
\end{table}

\subsection{Method for building an ego network of words \label{sec:building-egonet}}

%We call $\mathcal{W}(e)$ the multiset containing the sequence of words of a given ego $e$ obtained in the previous section. $\mathcal{W}_u(e)$  is the set containing the unique words of the same ego. 
Ego networks of words are used to hierarchise the words used by a given person based on their frequency. In the following, we summarise the model presented in~\cite{ollivier2022}. Let us focus on a tagged ego $e$ (hence, hereafter we drop the subscript $e$ in the notation). The ego network of words model is such that each word from $\mathcal{W}$ is assigned to one of $\tau$ rings $r_1$, $r_2$, $\ldots$ , $r_{\tau}$, knowing that $r_1$ (the innermost ring) contains the most frequently used words  and that $r_{\tau}$ (the outermost ring) contains the least used words. The set of words assigned to the ring $r_i$ is called $\mathcal{W}_{r_i}$ such that:
%
\begin{equation}
    %\begin{cases}
        %\mathcal{W}_u(e,r_i) \bigcap \mathcal{W}_u(e,r_j) = \emptyset, \forall i,j \in [1,\tau^{(e)}], i \neq j \\
        \mathcal{W} = \bigcup_{i=1}^{\tau} \mathcal{W}_{r_i}. %\\
        % |\,\mathcal{W}_u(e)\,| = \Sigma_{i=1}^{\tau^{(e)}} |\,\mathcal{W}_u(e,r_i)\,|
    %\end{cases}
    \label{eq:stability-eq1}
\end{equation}
%
% \begin{equation}
%         \mathcal{W} = \bigcup_{i=1}^{\tau} \mathcal{W}_{r_i}
%     \label{eq:stability-eq1}
% \end{equation}
%
The ego network can also be studied from a cumulative perspective with  concentric layers $l_1$, $l_2$, $\ldots$, $l_{\tau}$, with layer $l_i$ containing all the rings $r_j$ where $j \leq i$.  The set of words assigned to layer $l_i$ is denoted with $\mathcal{W}_{l_i}$, so:
%
\begin{equation}
    \mathcal{W}_{l_i} = \bigcup_{j=1}^{i} \mathcal{W}_{r_j}.
\end{equation}
%
This implies that the innermost layer $l_1$ is equivalent to $r_1$.
%and the outermost layer $l_{\tau}$ contains all the words of the ego network ($\mathcal{W}_{l_\tau} = \mathcal{W}$).

%In the following parts of the paper, we will refer to the circles (or layers) as $\mathcal{L}_i^{(e)}$ where $e$ is the corresponding ego network of word and $i$ the rank of the circle (from 1, the innermost circle to $\tau^{(e)}$ the outermost one). Since we will not use the time component in this study the frequency simply corresponds to the number of word occurrences. 
Words in an ego network are characterized by their usage frequency, which corresponds to their number of occurrences.
To find the best natural grouping of words (i.e., to find $\tau$) we use the Mean Shift~\cite{fukunaga1975estimation} algorithm, which is able, in contrast to Jenks~\cite{jenks1977optimal} or K-Means~\cite{macqueen1967some}, to automatically optimize $\tau$, the number of groups to be found. Clustering on a unidimensional variable is equivalent to dividing the word frequencies into mutually exclusive intervals.
The Mean Shift algorithm detects clusters that correspond to the local maxima of an estimated density function of word frequencies. This function is obtained with the kernel density estimation for which the sensibility is set with a fixed parameter called the bandwidth. We apply a preliminary log-transformation to frequencies in order to compress high values and ensure that the same bandwidth setting allows peak detection for both the high- and low-frequency parts of the distribution\footnote{Note that applying a log-transformation to word frequencies is common in psychological research when studying the associated cognitive processes~\cite{brysbaert2018word}.}.
The obtained clusters of words correspond to the $\tau$ rings of the newly built ego network of words for ego $e$, $r_1$ being the cluster containing the most frequent words and $r_{\tau}$ the one containing the least frequent words.

\subsection{Motivating the need for an active ego network extraction method}
\label{sec:full-egonet}

We start by applying the clustering algorithm to all the words in $\mathcal{W}_e$ for the egos in our datasets, and we plot the distribution of the number of circles $\tau$ in Figure~\ref{fig:nb-circles-full}. We can observe that the obtained ego networks of words have a very low number of circles (the most frequent case is two) compared with the ego networks of words in previous work (usually between five and seven circles~\cite{ollivier2020,ollivier2022}), despite exactly the same workflow being used. Note that the Twitter datasets used here are \emph{the same} as those in ~\cite{ollivier2020,ollivier2022} except for the timeline length considered (much larger, in this work). As we can observe in Figure~\ref{fig:occ-vs-layers}, ego networks with  one or two circles are also the biggest ego networks (\textit{i.e.} with the largest number of unique words $|\mathcal{W}|$). This seems to suggest that, when considering larger textual inputs, the ego network model loses its finer discriminative power. In fact, two-circle ego networks are considered uninteresting, as they simply separate the most used words from the least used words. 

However, this finding is not unexpected: in the social ego network case, the theory distinguishes between the \emph{full} and \emph{active} ego network, stating that only the relationships in the active part are actually consuming cognitive resources. The conventional cut-off point, as stated in \cite{dunbar1998social}, is for the social relationship to involve interactions at least once a year, which, in Western societies corresponds to at least exchanging Christmas/birthday wishes. While this cut-off point could be obtained with anthropological common sense for social ego networks, it is difficult to come up with a similar rule of thumb for the ego networks of words, which are less rooted in everyday experiences. Hence, in this work, we set out to design a methodology to automatically extract the cut-off point in the ego networks of words.



\begin{figure}[h]
\centering
\begin{minipage}{.48\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/nb-circles-full.pdf}\vspace{-8pt}
  \captionof{figure}{Distribution of the number of circles $\tau_{e}$}
  \label{fig:nb-circles-full}
\end{minipage} %
\hspace{5pt}
%
\begin{minipage}{.48\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/occ-vs-layers.pdf}\vspace{-8pt} % update figure 
  \captionof{figure}{Number of circles $\tau_{e}$ vs full ego network size ($|\,\mathcal{W}_e\,|$) in the MediaSum dataset. The same trend is observed in the other datasets (plots omitted to optimize the space).}
  \label{fig:occ-vs-layers}
\end{minipage}\vspace{-10pt}
\end{figure}

\subsection{Extracting the active ego network \label{sec:active-egonet}}

The idea behind an \emph{active} ego network is that all the words it contains should be actively used, even those in the outermost circle. If we let a person speak, we notice that from a certain point on %the frequency of appearance of a new word decreases rapidly:
the time between the appearance of two new words increases swiftly:
a specific number of words is sufficient for this person to express themself. This quantity is the maximum number of actively used words. We can observe this phenomenon in Figure~\ref{fig:saturation-curve1}, where we plotted the number of tokens needed to obtain an ego of a given size (which corresponds the number of unique words). 
%where the number of tokens $t$ (y-axis) vs the corresponding number of unique words $w$ (x-axis) is plotted for a single speaker in the Mediasum dataset. 
The curve is obtained by scanning the timeline (or, more exactly, the chronologically ordered tokens remaining after preprocessing the timeline) from start to end, and counting the new tokens and the unique words as we go. The catch is that not every new token corresponds to a new unique word. 
We will call this curve the \emph{saturation curve}, which we denote with $s$. Using the notation in Section~\ref{sec:preliminaries}, $s : |\mathcal{W}^n| \mapsto n$.

We can observe two regimes in Figure~\ref{fig:saturation-curve1}. In the first, the number of tokens grows slowly as new words are used, while in the second it grows faster. The rate at which new words are discovered is constant in both, but much higher in the first than in the second. If we approximate the curve in the two regimes with straight lines, the slope in the first regime is smaller than in the second. 
%
We argue that the active part of the ego network ends at the cut-off point of the saturation curve, i.e., where the first regime ends and the second one begins. The goal of this section is to describe a methodology for finding such point. The number of unique words at the cut-off point $\hat{w}$ of the curve corresponds to $|\mathcal{W}^{active}|$, while $max(w) = |\mathcal{W}|$ corresponds to $|\mathcal{W}^{full}|$, the total number of unique words in the ego network. If our intuition is confirmed, the well-known layered ego network structure would emerge by considering only words in the first regime of the saturation curve when computing the ego network. Indeed, we show this in Section~\ref{sec:cutoff-results}.
%
Note that sometimes the textual data for one ego is not large enough for the ego network to reach any cut-off point (Figure~\ref{fig:saturation-curve2}). In this case, there is no need to split the ego network into two parts.

%If we reach it, then we can just keep the corpus part needed to obtain that maximum number of active words. That is the rationale of the method explained in the next section.

\begin{figure}[h]
\centering
\begin{minipage}{.48\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/saturation-curve1.pdf}\vspace{-8pt}
  \captionof{figure}{Non-linear saturation curve.}
  \label{fig:saturation-curve1}
\end{minipage} %
\hspace{5pt}
%
\begin{minipage}{.48\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/saturation-curve2.pdf}\vspace{-8pt}
  \captionof{figure}{Linear saturation curve.}
  \label{fig:saturation-curve2}
\end{minipage}\vspace{-10pt}
\end{figure}

%First, the size of the ego network grows linearly, then after a bending point,  then the ego networks needs more and more word occurrences in the corpus to grow by one word.\\

\subsubsection{Methodology for identifying the cut-off point. \label{sec:methodology}}

We start with a high-level description of our methodology, illustrated in Figure~\ref{fig:methodology-recurs}. Let us focus on the curve~$t(w)$, and assume that it is not linear in $[0, \max(w)]$ (if it is linear, we can stop searching for the cut-off, since there is none). The idea is to split the curve at $\hat{w}$, such that there are two separate halves with different slopes. The search for $\hat{w}$ is done recursively, continuing to split the first half until it is effectively linear. 
At which point, the algorithm stops. The intuition is that the words and tokens before $\hat{w}$ correspond to the first regime described above, where new words are discovered at a higher rate.  

\begin{enumerate}
  \item If the saturation curve is linear
  \footnote{
  We use Lasso\cite{tibshirani1996regression} to determine if the curve described by $x_{[0,w_u]}$ and $y_{[0,w_u]}$ is linear. We define four polynomials features $<x_1,x_2,x_3,x_4>$ (degree one to degree four), reduced and centered, based on $x_{[0,w_u]}$. Additionally to the sum of square errors, Lasso adds a penalty $\lambda \Sigma_{i=1}^4 |\sigma_i|$ where $\lambda$ controls the impact of the penalty and $\sigma_i$ is the linear coefficient associated with $x_i$. Lasso has the particularity to reduce to 0 an increasing number of feature coefficients when $\lambda$ grows. It allows indirectly to select the best feature. If $\sigma_1$ is the last non-zero coefficient when $\lambda$ grows, it means that $x_1$ is the most suitable feature and thus the curve is linear.}
  %The objective function is $\min\limits_{\sigma} = \frac{1}{2 \times w_u} \Sigma_{i=1}^{4} || \sigma x - x_e[0,w_u] ||^2_2 - \lambda |\sigma|_1 $ where 
  on $[0,w_u^{full}]$ then the algorithm stops, the maximum number of active words is not reached ($w_u^{out} \gets W_u^{full}$). If not, the curve exhibits an inflection point that should be found.
  \item We select $w_u^{new}$ such that the sum of squares of two linear models fitted on intervals $[0,w_u^{new}]$ and $[w_u^{new},W_u^{full}]$ is the lowest.
  \item If the saturation curve is linear enough on $[0,w_u^{new}]$, then $w_u^{out} \gets w_u^{new}$. If not we repeat step 2 on interval $[0,w_u^{new}]$ to update $w_u^{new}$ with a lower value until $[0,w_u^{new}]$ is considered as linear.
  
\end{enumerate}


%%%%%%%%%%% OLD VERSION
The methodology to obtain the cut-off point $\mathcal{W}^{active}$ is illustrated in Figure~\ref{fig:methodology-recurs} and detailed in Algorithm~\ref{alg:cut-off}. 
To clarify the formulas in the following sections, we simplify the notation of the number of unique words in an ego network: $w_u = |\mathcal{W}_u(e)|$ at any point of the curve. For the ego network $e$, the two-dimensional coordinates of the curve on the interval $[0,w_u]$ are symbolized by $x_{[0,w_u]}$ and $y_{[0,w_u]}$.
%In Algorithm~\ref{alg:cut-off} the main function \textsc{FindCutOff} is recursive: if the saturation curve is linear 
Algorithm~\ref{alg:cut-off} describes how the cut-off point is found recursively:
\begin{enumerate}
  \item If the saturation curve is linear
  \footnote{
  We use Lasso\cite{tibshirani1996regression} to determine if the curve described by $x_{[0,w_u]}$ and $y_{[0,w_u]}$ is linear. We define four polynomials features $<x_1,x_2,x_3,x_4>$ (degree one to degree four), reduced and centered, based on $x_{[0,w_u]}$. Additionally to the sum of square errors, Lasso adds a penalty $\lambda \Sigma_{i=1}^4 |\sigma_i|$ where $\lambda$ controls the impact of the penalty and $\sigma_i$ is the linear coefficient associated with $x_i$. Lasso has the particularity to reduce to 0 an increasing number of feature coefficients when $\lambda$ grows. It allows indirectly to select the best feature. If $\sigma_1$ is the last non-zero coefficient when $\lambda$ grows, it means that $x_1$ is the most suitable feature and thus the curve is linear.}
  %The objective function is $\min\limits_{\sigma} = \frac{1}{2 \times w_u} \Sigma_{i=1}^{4} || \sigma x - x_e[0,w_u] ||^2_2 - \lambda |\sigma|_1 $ where 
  on $[0,w_u^{full}]$ then the algorithm stops, the maximum number of active words is not reached ($w_u^{out} \gets W_u^{full}$). If not, the curve exhibits an inflection point that should be found.
  \item We select $w_u^{new}$ such that the sum of squares of two linear models fitted on intervals $[0,w_u^{new}]$ and $[w_u^{new},W_u^{full}]$ is the lowest.
  \item If the saturation curve is linear enough on $[0,w_u^{new}]$, then $w_u^{out} \gets w_u^{new}$. If not we repeat step 2 on interval $[0,w_u^{new}]$ to update $w_u^{new}$ with a lower value until $[0,w_u^{new}]$ is considered as linear.
  
\end{enumerate}




%on interval $[0,\mathcal{W}_u^{full}]$, then the algorithm stops and the maximum number of active words is not reached ($w_u^{out} = W_u^{full} \leq W_u^{active}$). If not, we fit a two segments polyline (Algorithm~\ref{alg:break-point}) to detect two phases of the saturation curve and call \textsc{FindCutOff} again on the interval of first phase we just found. When that first phase is linear enough, we stop and consider that the saturation point is reached ($w_u^{out} = W_u^{active} < W_u^{full}$). 
%\footnote{In Algorithms \ref{alg:linear} and \ref{alg:break-point} we implicitly consider that the fitting are made on the saturation curve (\textit{i.e.} the x-axis being $w_u$ and the y-axis being $|\mathcal{W}(e)|$).} 
%We call $w_u^{sat}$ the number of unique words at the saturation point, and $w_u^{full}$ the number of unique words in the full ego network.

%\begin{enumerate}
%  \item Verify if the saturation curve is linear. If so, then the algorithm stops and the maximum number of active words is not reached ($w_u^{full} \leq w_u^{sat}$), jump to point four. If not, there is a saturation point to find ($w_u^{full} > w_u^{sat}$), we can jump to point two.
%  \item We divide the curve in two at point $w$ (a given number of unique words). We fit two linear models on both intervals $[0,w]$ and $[w,w_u^{sat}]$. We select $w$ such that the sum of squared errors of the composed model is the lowest.
%  \item We keep the first interval $[0,w]$ of the saturation curve and test if this part is linear enough (repeat step 1 with $w_u^{full} \gets w$).
%  \item We build the ego network whose size is $w_u^{out} \gets w_u^{full}$.
%\end{enumerate}

%\greybox{\textbf{Verifying if the saturation curve is linear}
%\begin{enumerate}
%    \item $w_u$: number of unique word, $|\,\mathcal{W}(e)\,|$: number of word occurrences
%    \item $<w_u^1, w_u^2, w_u^3, w_u^4>$ are the polynomial features, center and reduced.
%    \item Train a Lasso model, with a L1 penalty coefficient $\lambda$ as input, and four feature coefficients $\alpha_1$, $\alpha_2$, $\alpha_3$, $\alpha_4$ as output.
%    \item Select the feature $w_u^i$ with the last non-zero coefficient $\alpha_i$ when $\lambda$ grows.
%    \item If the feature is $w_u^1$, then we consider the saturation curve as linear.
%\end{enumerate}
%}

%We fit the curve with a linear combination of polynoms of degree 1, 2, 3 and 4.\\
%Use lasso to select the polynom degree that fits the best to the curve.\\
%If the 1 degree is the best fit, then we consider that it is linear \\
%If the curve is not linear, then we try to find the linear first phase

\begin{algorithm}
\caption{Find the cut-off point of the saturation curve}\label{alg:cut-off}

 \hspace*{\algorithmicindent} \textbf{Input: } $\mathbf{w} = \{w_i : w_i \in \mathcal{W}\}$ and $\mathbf{t} = \{t(w_i) : w_i \in \mathcal{W}\}$, i.e. the datapoints of the saturation curve \\
%  $x_{[0,w_u^{full}]}$ and $y_{[0,w_u^{full}]}$ the coordinates of the saturation curve of ego network $e$ on the interval $[0,w_u^{full}]$.\\
  \hspace*{\algorithmicindent} \textbf{Output: } $\hat{w}$, i.e. the cut-off point.\\
 %\hspace*{\algorithmicindent} \textbf{Output: } $w_u^{out}$ the cut-off point that delimits the active part of the saturation curve $[0,w_u^{out}]$\\

\begin{algorithmic}[1]
\State $\hat{w} \gets \Call{RecursiveCutOff}{\mathbf{w}, \mathbf{t}}$
\item[]
\Function{RecursiveCutOff}{$\mathbf{w}, \mathbf{t}$}
\If{\Call{IsLinear}{$\mathbf{w}, \mathbf{t}$}}
    \State \Return $\max(\mathbf{w})$
\Else
    \State $\hat{w} \gets $ \Call{FindPolylineBreak}{$\mathbf{w}, \mathbf{t}$}
    \State \Return \Call{RecursiveCutOff}{$\hat{w}$}
 \EndIf
\EndFunction
\item[]
%\caption{to check if the saturation is linear on interval $[0,w_u]$}\label{alg:linear}
\Function{IsLinear}{$\mathbf{w}, \mathbf{t}$}
    \State $\lambda \gets 0$ \Comment{Penalty coefficient of lasso regression}
    \State $<x_1,x_2,x_3, x_4>$ \Comment{Polynom. feat. based on $x_{[0,w_u^{new}]}$, center and reduced}
    \State $<\sigma_1, \sigma_2, \sigma_3, \sigma_4>$ \Comment{Lasso coefficient associated to the features}
    \State
    \While{\Call{CountNonZero}{$<\sigma_1, \sigma_2, \sigma_3, \sigma_4>$} $>1$}
        \State $\lambda \gets \lambda + \delta$
        \State $<\sigma_1, \sigma_2, \sigma_3, \sigma_4> \gets$ \Call{Lasso}{$x_{[0,w_u^{in}]}$,$y_{[0,w_u^{in}]}$,$<x_1,x_2,x_3,x_4>$,$\lambda$}
    \EndWhile
    \If{$\sigma_1 \neq 0$}
    \State \Return True
    \Else
    \State \Return False
    \EndIf
\EndFunction
\item[]
%\caption{to find the best break point of a 2-segments polyline fit}\label{alg:break-point}
\Function{FindPolylineBreak}{$w_u^{in}$}
    \State \Var{best_$w_u^{new}$} $\gets 1$
    \State \Var{lowest_ss} $\gets +\infty$
    \For{$w_u^{new} \in \llbracket 1,w_u^{in}-1 \rrbracket$}
        \State \Var{ss$_1$} $\gets$ \Call{LinearFit}{$x_{[0,w_u^{new}]}$,$y_{[0,w_u^{new}]}$}
        \State \Var{ss$_2$} $\gets$ \Call{LinearFit}{$x_{[w_u^{new},w_u^{in}]}$,$y_{[w_u^{new},w_u^{in}]}$}
        \If{\Var{ss$_1$}+\Var{ss$_2$}$<$\Var{lowest_ss}}
            \State \Var{lowest_ss} $\gets$ \Var{ss$_1$}+\Var{ss$_2$}
            \State \Var{best_$w_u^{new}$} $\gets$ $w_u^{new}$
        \EndIf
    \EndFor
    \State \Return \Var{best_$w_u^{new}$}
\EndFunction
\end{algorithmic}
\end{algorithm}

\begin{figure}[h]
    \begin{center}
        \includegraphics[scale=.4]{figures/methodology-recurs.pdf}%\vspace{-5pt}
        \caption{Algorithm for detecting the saturation point.}
        \label{fig:methodology-recurs}\vspace{-30pt}
    \end{center}
\end{figure} 

\subsection{Stability \label{sec:stability}}

The approximation of the size of the active ego network $W_u^{active}$ should be stable over time and specific to each person. 
%It means that on a theoretical infinite saturation curve, \textsc{FindCutOff}($[0,w_u^{in}]$) should return $w_u^{out}=w_u^{in}$ when $w_u^{in} \in [0,W_u^{active}]$ and $w_u^{out}=W_u^{active}$ when $w_u^{in} \in [W_u^{active},+\infty]$.
It means that on a theoretical infinite saturation curve, \textsc{RecursiveCutOff}($w_u^{in}$) should return $w_u^{out}=W_u^{active}$ when $w_u^{in} \geq W_u^{active}$. In this case, we can approximate $W_u^{active}$ with $w_u^{out}$. When $w_u^{in} < W_u^{active}$ (which is the case where the saturation curve has no inflection point), the algorithm shall simply return $w_u^{out} = w_u^{in}$. 

%if we had calculated the saturation curve with more words (\textit{i.e.} a bigger $|\,w_u^{full}\,|$), the bending point should remain the same. We want to verify if our algorithm verifies that stability constraint. 
To prove that our algorithm respects that ideal behaviour, we first calculate $W_u^{out}$ the output of the algorithm calculated with the full curve of a given user:
\begin{equation}
    W_u^{out} \gets \CUTOFF(W_u^{full})
\end{equation}
If the curve contains a saturation point, then $W_u^{out} = W_u^{active}$, if not then $W_u^{out} < W_u^{active}$.
%, and $y_{sat}$ and the size of the corpus (number of word occurrences) needed obtain $x_{sat}$ unique words. 
%We select a subpart of the curve in the interval $[0,x_{in}]$ as input to our algorithm, and we obtain an estimation of saturation point at $x_{out}$. In the ideal case, $x_{out}$ should follow the behaviour:
%\begin{equation}
%    \begin{cases}
%        w_u^{out}=w_u^{in} \;\;\;\text{for}\;\;\;  \in [0,w_u^{sat}] \\
%        w_u^{out}=w_u^{sat} \;\;\;\text{for}\;\;\; x \in [x_{sat},+\infty]
%    \end{cases}
%    \label{eq:stability-eq1}
%\end{equation}
In order to compare the results obtained with various scales, we use the ratio $\frac{w_u^{out}}{W_u^{out}}$. As stated above $w_u^{out}$ should verify the following conditions:

\begin{equation}
    \begin{cases}
        \cfrac{w_u^{out}}{W_u^{out}}=\cfrac{w_u^{in}}{W_u^{out}} \;\;\;\text{when}\;\;\; \cfrac{w_u^{in}}{W_u^{out}} \in [0,1]\\
        \cfrac{w_u^{out}}{W_u^{out}}=1 \;\;\;\text{when}\;\;\; \cfrac{w_u^{in}}{W_u^{out}} \in [1,+\infty]
    \end{cases}
    \label{eq:stability-eq2}
\end{equation}

We confirm with the empirical results in Fig~\ref{fig:stability} that the behavior of the algorithm is close to the ideal case in every dataset despite some noise due to a lower number of ego networks in the NYT journalists and science writers dataset.
%We can observe a little bump when $\cfrac{x_{out}}{x_{sat}}$ is slightly superior to $1$. We can explain this phenomenon because because we feed the algorithm with the saturation curve at between the interval $[0,x_{sat}+\epsilon]$. On this interval, the saturation curve only starts its inflexion, which is not yet detected. Once $\epsilon$ and the second phase is large enough to be detected, the algorithm gets very close to the ideal case.

\begin{figure}[h]
    \begin{center}
        \includegraphics[scale=.35]{figures/stability}%\vspace{-5pt}
        \caption{The stability of the algorithm is close from the ideal case.}
        \label{fig:stability}
    \end{center}
\end{figure} 

\subsection{Temporal stability of the active network size \label{sec:temporal-stability}}

The temporal evolution of the size of the active network is important because it allows us to measure if the cognitive ability to add words to one's active vocabulary evolves over time. To evaluate the temporal evolution of this value, we change the starting index of the sequence of words $w_0,w_1,\cdots,w_n$ from which we build the saturation curve. This shift $\delta$ in the considered word sequence does not correspond to a proper time unit, but to the number of words skipped, such that the new word sequence is $w_\delta,w_{\delta+1},\cdots,w_n$. Based on this updated sequence of words, we build a new saturation curve, from which we extract an active network size $W_u^{active}(\delta)$ (Figure~\ref{fig:temp-shift-stability-method}). Since the size of the word sequence varies depending on the ego network, a too-big $\delta$ would reduce it enough to make it impossible to build a curve containing the whole of its active part (\textit{i.e.} a curve with a bending point). For each ego network, we define $\delta_{max}$ which leaves a minimum number of words $n-\delta_{max}$ in the sequence. That number corresponds to the minimum size of the word sequence needed to find $W_u^{active}(0)$ for $\delta = 0$. In Figure~\ref{fig:temp-shift-stability-res}, we choose a $\delta$ range from 0 to $5 \cdot 10^4$. That maximum was chosen because it is the largest value for which at least 25\% of the ego network has a $\delta_{max}$ higher than it. In this way, we keep the largest interval over which we can obtain meaningful results. We can observe in Figure~\ref{fig:temp-shift-stability-res} that the size of the active ego network is stable when $\delta$ grows, independently of the dataset. This legitimizes our hypothesis that the size and internal structure of the ego network are bound by cognitive constraints that are applied at different intensities depending on the individual, but which are themselves stable over time. Now that these results are confirmed, all the following results are obtained from the complete word sequence (\textit{i.e.} $\delta=0$).

\begin{figure}[h]
    \begin{center}
        \includegraphics[scale=.6]{figures/temp-shift-stability-method.pdf}%\vspace{-5pt}
        \caption{The diagram illustrates the temporal analysis procedure of the active size of an ego network. A temporal change corresponds here to a change in the index $\delta$ of the first word of the sequence used to build the ego network. This change leads by construction to a different saturation curve from which we will extract and study the variability of the active part size $W_u^{active}(\delta)$.}
        \label{fig:temp-shift-stability-method}
    \end{center}
\end{figure} 

\begin{figure}[h]
    \begin{center}
        \includegraphics[scale=.6]{figures/temp-shift-stability-res.pdf}%\vspace{-5pt}
        \caption{The shift $\delta$ of the word sequence from which the ego networks are built has almost no influence on the active size $W_u^{active}(\delta)$ on. In order to average that behaviour at the dataset level, we consider the ratio $\frac{W_u^{active}(\delta)}{W_u^{active}(0)}$ where the divisor is the original active size at $\delta=0$. This ratio is consistently close to one (the maximum average value is $1.25$, reached by the MediaSum dataset for $\delta=5 \times 10^5$). These aggregated values are reliable since the 95\% average confidence interval is only $\pm0.08$}
        %The interval $0 \leq \delta \leq 5 \times 10^5$.}
        \label{fig:temp-shift-stability-res}
    \end{center}
\end{figure} 

\subsection{Results \label{sec:cutoff-results}}

The distribution of circles of the newly built ego networks of words can be seen in Fig~\ref{fig:nb-circles-active}. Limiting the size of the ego network to the maximum number of actively used words shifts the mode from two circles to four and five circles, for all datasets. These results validate our methodology. In the next section, we will study the structural properties of these ego networks of words.

\begin{figure}[h]
    \begin{center}
        \includegraphics[scale=.5]{figures/nb-circles-active.pdf}%\vspace{-5pt}
        \caption{Effects of the recursive cut on the distribution of the number of circles.}
        \label{fig:nb-circles-active}
    \end{center}
\end{figure} 
